Adjoint-based optimization of the control boundaries of a microfluidic acoustic flow

In this study, we find the optimal control boundary (i.e., actuator velocity) that cancels the acoustic reverberations inside drop-on-demand inkjet printheads at a specific time. We formulate an optimization problem to minimize the total energy of the oscillating flow at a given time (i.e., the acoustic energy inside the microchannel and the surface energy of the droplet). We use the adjoint method to compute the gradient of the cost function with respect to the control boundary, and a gradient-based optimization algorithm to converge to the optimal solution. This methodology has been successfully applied to two generic inkjet printhead mechanisms: thin-film and bulk types. In both cases, the actuator first reduces the surface energy of the system by extracting fluid from the nozzle. In this process, acoustic waves also propagate through the channel and reverberate at the ends, which increases the acoustic energy of the system. The actuator then sends additional acoustic waves that cancel these reverberations. Both mechanisms have been able to reduce the total energy of the system by a factor of over 100 in comparison with the uncontrolled cases.

==> references.tex <==
@Preamble{ " \newcommand{\noop}[1]{} " }




@phdthesis{Geiyer2017,
    author     =     {Daniel Geiyer},
    title     =     {{Chaotification as a Means of Broadband Vibration Energy Harvesting with Piezoelectric Materials}},
    school     =     {University of Central Florida},
    address     =     {Orlando, Florida},
    year     =     {2017},
    note = {Doctoral Dissertation. Electronic Theses and Dissertations. no 5692. \url{http://stars.library.ucf.edu/etd/5692}},
    }


@article{kungurtsev_juniper_2019, 
title={Adjoint-based shape optimization of the microchannels in an inkjet printhead}, 
volume={871}, 
DOI={10.1017/jfm.2019.271}, 
journal={Journal of Fluid Mechanics}, 
publisher={Cambridge University Press}, 
author={Kungurtsev, Petr V. and Juniper, Matthew P.}, 
year={2019}, 
pages={113–138}}


@article{Kungurtsev2023,
title = {{Adjoint-based optimization of the actuator velocity profile in an inkjet print head}},
author = {Kungurtsev, P. and Juniper, M. P.},
year= {2023},
journal = {Eur. J. Mech. B. (Fluids) (accepted)},
volume = {},
pages = {},
}


@article{LEE201185,
title = {Silver nanoplates as inkjet ink particles for metallization at a low baking temperature of 100°C},
journal = {Colloids and Surfaces A: Physicochemical and Engineering Aspects},
volume = {381},
number = {1},
pages = {85-91},
year = {2011},
issn = {0927-7757},
doi = {https://doi.org/10.1016/j.colsurfa.2011.03.034},
url = {https://www.sciencedirect.com/science/article/pii/S0927775711001981},
author = {Chien-Liang Lee and Kun-Chuan Chang and Ciou-Mei Syu},
keywords = {Inkjet printing, Sintering, Silver, Nanoparticle, Electroless},
abstract = {Conductive patterns on a flexible polyimide film using Ag nanoplate ink of 10wt% solid content were successfully fabricated by inkjet printing and baking at a low temperature of 100°C. Sintering on these printed nanoplates at a low temperature (100°C) led to the formation of connections between nanoplates. A four-point probe measurement indicated that the resistivity of the line obtained by printing nanoplates is 26.3μΩ-cm and this is lower than that of the line obtained by printing spherical nanoparticles, 4.3×105μΩ-cm.}
}

@article{tomaszewski2017drops,
  title={Drops forming in inkjet printing of flexible electronic circuits},
  author={Tomaszewski, Grzegorz and Potencki, Jerzy},
  journal={Circuit World},
  year={2017},
  publisher={Emerald Publishing Limited}
}

@article{chiolerio2014inkjet,
  title={Inkjet printed negative supercapacitors: synthesis of polyaniline-based inks, doping agent effect, and advanced electronic devices applications},
  author={Chiolerio, Alessandro and Bocchini, Sergio and Porro, Samuele},
  journal={Advanced Functional Materials},
  volume={24},
  number={22},
  pages={3375--3383},
  year={2014},
  publisher={Wiley Online Library}
}


@article{Lorber_2013,
	doi = {10.1088/1758-5082/6/1/015001},
	url = {https://doi.org/10.1088/1758-5082/6/1/015001},
	year = 2013,
	month = {dec},
	publisher = {{IOP} Publishing},
	volume = {6},
	number = {1},
	pages = {015001},
	author = {Barbara Lorber and Wen-Kai Hsiao and Ian M Hutchings and Keith R Martin},
	title = {Adult rat retinal ganglion cells and glia can be printed by piezoelectric inkjet printing},
	journal = {Biofabrication},
	abstract = {We have investigated whether inkjet printing technology can be extended to print cells of the adult rat central nervous system (CNS), retinal ganglion cells (RGC) and glia, and the effects on survival and growth of these cells in culture, which is an important step in the development of tissue grafts for regenerative medicine, and may aid in the cure of blindness. We observed that RGC and glia can be successfully printed using a piezoelectric printer. Whilst inkjet printing reduced the cell population due to sedimentation within the printing system, imaging of the printhead nozzle, which is the area where the cells experience the greatest shear stress and rate, confirmed that there was no evidence of destruction or even significant distortion of the cells during jet ejection and drop formation. Importantly, the viability of the cells was not affected by the printing process. When we cultured the same number of printed and non-printed RGC/glial cells, there was no significant difference in cell survival and RGC neurite outgrowth. In addition, use of a glial substrate significantly increased RGC neurite outgrowth, and this effect was retained when the cells had been printed. In conclusion, printing of RGC and glia using a piezoelectric printhead does not adversely affect viability and survival/growth of the cells in culture. Importantly, printed glial cells retain their growth-promoting properties when used as a substrate, opening new avenues for printed CNS grafts in regenerative medicine.}
}

@book{hoath2016fundamentals,
  title={Fundamentals of inkjet printing: the science of inkjet and droplets},
  author={Hoath, Stephen D},
  year={2016},
  publisher={John Wiley \& Sons}
}

@article{wright1999numerical,
  title={Numerical optimization},
  author={Wright, Stephen and Nocedal, Jorge and others},
  journal={Springer Science},
  volume={35},
  number={67-68},
  pages={7},
  year={1999}
}
